Cache Me If You Must: Adaptive Key-Value Quantization for Large Language Models

Efficient real-world deployments of large language models (LLMs) rely on Key-Value (KV) caching for processing and generating long outputs, reducing the need for repetitive computation. For large contexts, Key-Value caches can take up tens of gigabytes of device memory, as they store vector representations for each token and layer. Recent work has shown that the cached vectors can be compressed through quantization, pruning or merging, but these techniques often compromise quality towards higher compression rates. In this work, we aim to improve Key & Value compression by exploiting two observations: 1) the inherent dependencies between keys and values across different layers, and 2) high-compression mechanisms for internal network states. We propose AQUA-KV, an adaptive quantization for Key-Value caches that relies on compact adapters to exploit existing dependencies between Keys and Values, and aims to "optimally" compress the information that cannot be predicted. AQUA-KV significantly improves compression rates, while maintaining high accuracy on state-of-the-art LLM families. On Llama 3.2 LLMs, we achieve near-lossless inference at 2-2.5 bits per value with under $1\%$ relative error in perplexity and LongBench scores. AQUA-KV is one-shot, simple, and efficient: it can be calibrated on a single GPU within 1-6 hours, even for 70B models.

==> resources/tables/longbench_results_qwen-2.5-instruct.tex <==
\begin{table}[htb]
\footnotesize
\centering
\setlength\tabcolsep{3pt}
\caption{Evaluation of different KV cache compression methods on LongBench for Qwen-2.5 model family.}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\textbf{Model} & \textbf{Configuration} & \textbf{Avg bits} & \textbf{Avg LongBench} \\
\multirow{4}{*}{3B-Instruct} & fp16 & 16 & 31.61 \\
\cmidrule{2-4}
& AQUA-KV & 
\midrule
\multirow{5}{*}{7B-Instruct} & fp16 & 16 & 39.14 \\
\cmidrule{2-4}
\midrule
\bottomrule
\end{tabular}
\label{tab:llama2-depth-table}
}
\end{table}

